{\DH}Archer: Detecting On-Chain-Off-Chain Synchronization Bugs in Decentralized Applications

Since the emergence of Ethereum, blockchain-based decentralized applications (DApps) have become increasingly popular and important. To balance the security, performance, and costs, a DApp typically consists of two layers: an on-chain layer to execute transactions and store crucial data on the blockchain and an off-chain layer to interact with users. A DApp needs to synchronize its off-chain layer with the on-chain layer proactively. Otherwise, the inconsistent data in the off-chain layer could mislead users and cause undesirable consequences, e.g., loss of transaction fees. However, transactions sent to the blockchain are not guaranteed to be executed and could even be reversed after execution due to chain reorganization. Such non-determinism in the transaction execution is unique to blockchain. DApp developers may fail to perform the on-chain-off-chain synchronization accurately due to their lack of familiarity with the complex transaction lifecycle. In this work, we investigate the challenges of synchronizing on-chain and off-chain data in Ethereum-based DApps. We present two types of bugs that could result in inconsistencies between the on-chain and off-chain layers. To help detect such on-chain-off-chain synchronization bugs, we introduce a state transition model to guide the testing of DApps and propose two effective oracles to facilitate the automatic identification of bugs. We build the first testing framework, DArcher, to detect on-chain-off-chain synchronization bugs in DApps. We have evaluated DArcher on 11 popular real-world DApps. DArcher achieves high precision (99.3%), recall (87.6%), and accuracy (89.4%) in bug detection and significantly outperforms the baseline methods. It has found 15 real bugs in the 11 DApps. So far, six of the 15 bugs have been confirmed by the developers, and three have been fixed. These promising results demonstrate the usefulness of DArcher.

==> 4-Methodology/methodology-v1.tex <==
\subsection{On-Chain-Off-Chain Synchronization Bug}\label{subsec:on-chain-off-chain-synchronization-bug}
In Section~\ref{sec:motivating-example}, we present an example of an on-chain-off-chain synchronization bug residing in a popular DApp.
This type of bugs has not been studied in existing literature.
This section discusses the cause and consequence of such bugs, as well as the challenges to detect them.

A transaction may make an update on the on-chain state of a DApp.
Such a transaction, if successful, should lead to corresponding modification of the DApp's off-chain state, when the on-chain-off-chain synchronization is properly performed. 
Although the on-chain and the off-chain states need to be consistent, they are not necessarily identical. 
For instance, in the motivating example, Giveth's cache server processes on-chain donations and stores structured data, instead of making a copy of the on-chain state, as the off-chain state is to facilitate front-end enquiries.
In most situations, it is suffice for an off-chain state to keep a simplified view of the corresponding on-chain state to facilitate front-end user actions.

We introduce some terminologies to facilitate the illustration.
To model this criterion as a test oracle, we use $\mu(t,s)$ and $\sigma(t,s)$ to denote a DApp's on-chain and off-chain state in transaction $t$ at lifecycle state $s$, respectively. 
Note that a transaction can stay at each lifecycle state for a period of time, and a DApp may change its off-chain state during the period, $\sigma(t,s)$ refers to DApp's last off-chain state value when $t$ is at $s$.
In addition, as a transaction can visit \PendingState and \ExecutedState multiple times, we use $\mu_i(t,s)$ and $\sigma_i(t,s)$ to denote the on-chain and off-chain state, respectively, when $t$ makes the $i^{th}$ visit of \PendingState or \ExecutedState state, i.e., in the case where $s$ is either \PendingState or \ExecutedState. %\scc{We should introduce notations close to the place where we use them. Better move the last sentence to Oracle 1. Strictly speaking, $\sigma(t,s)$ is ambiguous because t can stay at s for a period of time during which the off-chain state may have changed from one value to another. So, which off-chain state value does $\sigma(t,s)$ refer to? I think we implicitly use $\sigma$ to refer to the last value but have not explained it clearly.} \aaron{I have clarified that we use the last value of off-chain state when transaction is at each lifecycle state.}

% The design of test oracles imposes another challenge in detecting on-chain-off-chain synchronization bugs.
% So it is hard to determine whether an off-chain state has been synchronized with an on-chain state by checking whether they have the same content. 

Let $f$ denote the mapping between the on-chain and the off-chain states. The following assertion governs the consistency between the on-chain and off-chain states when a transaction starts or reaches the end of its lifecycle, i.e.,\ initial and terminal states. 

\begin{consistency}
    For each transaction $t$, $\forall s \in \{\CreatedState,\DroppedState, \ConfirmedState\}$, $\sigma(t,s) = f(\mu(t,s))$
\end{consistency}

%It is tolerable that on-chain and off-chain states are temporarily inconsistent before the lifecycle ends. 
If this assertion is violated, we consider that a on-chain-off-chain synchronization bug exists in the DApp. Transient inconsistency is tolerated before the lifecycle ends.

% \begin{figure*}
%     \centering
%     \includegraphics{4-Methodology/bugs.pdf}
%     \caption{Transaction Lifecycles for the Two Types of On-Chain-Off-Chain Synchronization Bugs. Solid arrows show the actual transitions, and dashed arrows show the non-existent transitions assumed by DApps. For Type-I bugs, the off-chain state is prematurely updated when the transaction is \PendingState. For Type-II bugs, the off-chain state is updated when the transaction is \ExecutedState, but the updated state is not reverted when the transaction is later reversed.%\scc{Do not use yellow color. The green color does not stand out. Use dashed arrows for non-existent transitions assumed by DApp. The figures should make sense even reviewers/readers read it using hard copies. Quite a few reviewers who I know review papers using hard copies. Add the explanation of the notations in the caption. Can even put the explanation of the meaning of the figures in the caption.}
%     }
%     \label{fig:bug-diagram}
% \end{figure*}

%The performance bottleneck makes developers of DApps have to separate DApp into \textit{on-chain layer} and \textit{off-chain layer}, where the data stored are called \textit{on-chain state} and \textit{off-chain state} respectively.
%Off-chain state is not necessarily a cache but more often an application-level abstraction of the on-chain state, since storing data on chain is very expensive and with high latency.
%Therefore, the consistency between on-chain state and off-chain state is essential.
As discussed, it is essential to keep the consistency between the on-chain state and off-chain state of a DApp.
DApp users often take actions and prepare the required transaction arguments based on a DApp's off-chain state (i.e., the information that can be perceived from the front-end client).
Inconsistencies between DApp's off-chain state and on-chain state can result in losing transaction fees and making irreversible changes on blockchain.
%If DApps perform actions based on an off-chain state inconsistent with on-chain state, DApps may end up with poor user experience by showing incorrect information to users, or even sending subsequent transactions containing invalid data, losing transaction fees or making irreversible changes on blockchain.
%To mitigate these potential risks, a DApp needs to be tested for its on-chain-off-chain synchronization.
% We refer to the process of keeping consistency as \textit{on-chain-off-chain synchronization}, which is complicated because of the non-deterministic state transition in transaction lifecycles. 
%\scc{Should we more concretely emphasize the complication arises from the existence of the \PendingState state where (1) the transaction may be rejected and (2) it can be revisited instead of non-determinism, which is a more general concept? The existence of the \PendingState and its possible outcomes are not considered by existing testing techniques. The explanation using lifecycle non-determinism is a bit vague and cannot precisely point to the limitation of existing testing techniques.}
%\aaron{We emphasize the limitation of existing techniques after Type-II bugs.}
We categorize the on-chain-off-chain synchronization bugs into two types according to the two different causes of inconsistencies between on-chain and off-chain state.
\subsubsection{Type-I Bugs}
Type-I bugs are those that cause inconsistencies where a DApp's off-chain state is updated as if the transaction has been successfully executed while it is still at \PendingState state awaiting execution in the mining pool. 
The transaction could transit from the \PendingState to \DroppedState state later, instead of getting executed.
Fig.~\ref{fig:bug-diagram}(a) illustrate the case where Type-I bug occurs. 
A DApp's off-chain state is prematurely updated when a transaction is sent (i.e.,\ at \PendingState state).
The DApp assumes that the transaction would go through the dashed arrow path and updates its off-chain state as if the transaction is executed.
However, the transaction is actually dropped instead of executed. 
Since the on-chain state is not updated by the dropped transaction, premature update on off-chain state induces inconsistencies with on-chain states. 
%Inconsistencies between on-chain and off-chain state may occur when developers prematurely assume transactions are successful once they are sent. 
%\scc{Should we introduce Fig. 3(a) here?}
%An DApp's on-chain state has not been modified when its transaction is at the \PendingState state.
%If the off-chain state is prematurely updated at this state, inconsistencies can be induced.
%In addition, it is impossible to know whether a transaction execution will succeed or fail, and on-chain state will not change if the transaction is executed with a failure. 
%So it is unsafe to update off-chain state when a transaction is in \PendingState state.
%\scc{Are the last three sentences too repetitive? 110 and 112 deliver similar argument. 113 seems irrelevant. 114 repeats the argument again.}
%\aaron{I think so. I just want to explain the case that transaction fails. So delete 111-114?} \scc{I think the sentences can be deleted. 108 already suggests that the assumption could be wrong, including "successfully executed".} 
%\scc{Should it be successfully instead of instantly? If the bugs include pre-mature updates of the off-chain state for failing transactions, we need to explain how this could happen. By the way, if we are not referring to specific transactions, we should not say ``the transactions''. Use ``the'' carefully.}
%\aaron{I think if the transaction will succeed, the off-chain state shouldn't be updated at \PendingState state. And if the transaction will fail, the off-chain state should not be updated as well, since a failing transaction will not make any change on the on-chain state. So I think we don't need to mention whether developers assume transactions are executed successfully or not.} \scc{I could not follow the explanation. Any illustration? So, what do the developers update when the bugs occur? Do the developers update the off-chain state as if the transaction has been executed successfully? Here, we say that the bugs occur when developers have made the update. So, what have they updated to the off-chain state?}
%\aaron{Yes, if Type-I bugs occur, developers usually update off-chain state as if the transaction is executed successfully. } \scc{This is my point. So, we should explain it clearly.}

\subsubsection{Type-II Bugs}
A type-II bug occurs if a DApp updates the off-chain state when a transaction is executed, but does not revert when the transaction is reversed at the on-chain layer due to chain reorganization. %\scc{I rephrase the sentence ``Type-II bugs occur when DApp's off-chain state indicates ...'' because the original sentence does not accurately deliver the meaning.}
%Even if a DApp is aware of the existence of transaction \PendingState and does not suffer from Type-I bugs, the existence of 
The possibility of transiting from the \ExecutedState to \PendingState state can induce inconsistencies, because the result of a transaction execution is volatile before it has enough confirmations.
% \aaron{Previously in background we didn't introduce ``confirmation''. In lifecycle model, we also don't mention ``confirmation''. Should I introduce it now in background?} \scc{Yes, we can explain it when we discuss chain reorganization.}\aaron{Explained in background}
Fig.~\ref{fig:bug-diagram}(b) illustrates the case where Type-II bug occurs.
A DApp updates its off-chain state when a transaction is executed (i.e.,~at \ExecutedState state). 
The DApp assumes the transaction would reach \ConfirmedState state, but it actually gets reversed due to chain reorganization. 
The DApp does not revert the off-chain state, and if the reversed transaction is later dropped, inconsistencies between the on-chain and off-chain states are induced. 
% Type-II bugs often occur when developers are not aware of the existence of chain reorganization, which is a unique characteristic specific to blockchain.
%\scc{Should we introduce Fig 3(b) here?}

\subsection{Testing On-Chain-Off-Chain Synchronization}\label{subsec:oracles}

The existence of \PendingState state and the transition to \DroppedState state make it challenging for developers to assure proper on-chain-off-chain synchronization, while maintaining timely responses to user requests.
It requires developers to carefully handle two cases, where (1) a sent transaction could be dropped silently by the blockchain, and (2) an executed transaction could be reversed due to unexpected chain reorganization and become \PendingState again. 
The synchronization bugs arising from these two cases, which are unique to blockchain transactions, have not been considered by existing test methodologies and facilities.

%The detection of the synchronization bugs such arise cannot be effectively detected using existing test methodologies and facilities.
\lili{I feel that we'd better not say the existing test methodology and facilities do not consider the synchronization between on-chain and off-chain layers since we do not have any further illustrations on this argument. I instead just explain that the commonly-used testing environments do not consider all the possible transitions in transaction lifecycle transitions.} 
\aaron{OK} %\scc{To be picky, better to point out the limitations that \darcher addresses because (1) the lifecycle may not have modeled all possible transitions of a transaction and (2) \darcher may not have considered the testing of all possible transitions. The lifecycle is already a contribution by modeling some states and transitions that have not been considered in the literature. The lifecycle does not need to be comprehensive and we do not need to claim that it is comprehensive.}
%\aaron{I add one more paragraph in this subsection, explaining how \darcher address the limitations.}
% which do not consider the synchronization between the off-chain and the on-chain layers in a transaction lifecycle. %it is not easy to test on-chain-off-chain synchronization bugs using existing test utilities.
%The interactions between off-chain and on-chain layer must be considered in the testing.
%Testing only on off-chain layer of DApps can hardly reveal on-chain-off-chain synchronization bugs since transaction execution is not involved. %\scc{Why? A DApp comprises both off-chain and on-chain layers. Unit tests of the withdrawDonation() are supposed to enact both layers. If so, why can't unit tests reveal synchronization bugs? Are we making additional assumptions on unit testing?}\aaron{I should write ``testing only on off-chain layer'' here. It is similar to the argument we wrote in the DInfra proposal. }
%On-chain-off-chain synchronization must be involved in the testing such that the bug can be revealed.
%\scc{I revised the wording to make the argument more focused, more precise (I hope), less repetitive, less controversial and less writing mistakes.}
%Commonly-used blockchain testing environments execute transactions without visiting all the possible transitions in transaction lifecycles.
%As a result, they cannot detect the synchronization bugs that arise due to the non-determinism in transaction lifecycles. 
%\scc{To be picky, \darcher may not have considered the testing of all possible transitions. It is already a contribution by traversing some states and transitions that have not been considered in the literature. We do not need to claim that \darcher tests the lifecycle comprehensively. As such, it is inappropriate to criticize existing techniques for the same reason. We can be more specific in the criticism. Indeed, I think the last two sentences are redundant.} 
%\aaron{I delete them. They are indeed redundant. Without the last two sentences, I think we do not criticize that existing techniques do not consider all possible transitions. The following sentences should only point out the limitation that \darcher solves.}
%  in on-chain-off-chain synchronization in that the transaction execution on them is deterministic, eliminating the occurrence prerequisites of \bug.
%\scc{What is end-to-end testing. How is it different from unit testing, say for the withdrawDonation()?}\aaron{I found developers usually use ``end-to-end'' testing in the tests they wrote. It refers to the tests that go through the entire workflow of DApp from front-end (UI) to back-end (smart contracts). I think we can use ``integrated test'' instead.}
% This involves the interactions between DApps and blockchain but it is still hard to simulate a non-deterministic scenario of transaction execution.
%\scc{The presented argument of unit testing and end-to-end testing is a bit ad hoc. Maybe we can refer to the withdrawDonation() to clarify our argument. For example, why couldn't the unit tests of withdrawDonation() cannot reveal the synchronization bug even they involve both the on-chain and off-chain layers. It seems to me that the inadequacy arises from available test facilities rather but we present the inadequacy as the limitation of unit tests.}
%\aaron{I rephrase the argument to emphasize the inadequacy of testing facilities. We have already discuss the limitation of existing test environments using the motivating example in Section~\ref{sec:motivating-example}, I think there is no need to discuss the example again.}
Specifically, existing blockchain test environments, e.g.,\ Ganache\footnote{https://www.trufflesuite.com/ganache}, use a single miner in a private blockchain.
As a result, transactions are executed once they are sent. The \PendingState state in the transaction lifecycle essentially does not exist. %guaranteed to be executed and confirmed instantly on such blockchain test environments.
% Furthermore, transactions sent to blockchain are guaranteed to be executed instantly.
There are no chances for these transactions to be dropped after pending or reversed after execution.
On-chain-off-chain synchronization bugs induced by the aforementioned two cases can thus easily escape from testing. 

To address the limitation, %s that some of transaction state transitions are not covered in the testing,
\darcher implements a blockchain environment that allows control on the transaction lifecycle states.
Instead of executing a transaction immediately after sent, \darcher drives the transaction to make possible transitions that are neglected by existing blockchain testing environments at the \PendingState and \ExecutedState states, so that on-chain-off-chain synchronization bugs can be revealed.

% since no blockchain reorganization could happen with one miner.
\lili{I think the problem is not that the transactions are executed deterministically. The problem is that they do not simulate all the possible lifecycle state transitions. 
To effectively detect on-chain-off-chain synchronization bugs, we propose \darcher.}
\aaron{I agree, I think the current statements are better?}

%Using such a blockchain without non-deterministic transaction execution, it is hard to reveal on-chain-off-chain synchronization bugs.
% In the motivating example we discussed in Section~\ref{sec:motivating-example}, Giveth uses Ganache as development environment to test the DApp.
% The donation withdraw transaction will be executed immediately when it is received by blockchain, and it will never be revoked.
% There will be only a very short period of time when the transaction stays at \PendingState state, and there is nearly no difference whether the update of off-chain state is performed at \PendingState or \ExecutedState state.
% It is also impossible for the transaction to be revoked so it is safe to consider it to be finalized after execution.
% As a result, \bugs can hardly be revealed even if it exists when developers are using existing testing blockchain environments.

The design of test oracles imposes another challenge in detecting on-chain-off-chain synchronization bugs.
Evaluating the aforementioned consistency assertion is impractical in automatic testing of DApps. 
The mapping between the on-chain and the off-chain states is specific to each DApp.
It is hard to determine without related specification from developers.
% This imposes a technical challenge to deciding whether a DApp performs on-chain-off-chain synchronization correctly.
% It is hard to automatically decide how off-chain state is expected to update when transaction lifecycle state transits from one to another.
\lili{Shall we add a few sentences to illustrate why it is tricky to determine if a DApp performs on-chain-off-chain synchronization properly?}
\aaron{I add one more sentence, but I cannot justify it using existing works or other proofs.}

%\aaron{I don't think we can claim transactions sent from a DApp are executed sequentially. Each transaction's lifecycle can overlap with each other temporally. In the implementation of \darcher I isolate each transaction and make it sequential.} \scc{Like concurrent database transactions, are the transactions serializable? If so, we can analyze each transaction in isolation? I meant such analysis does not introduce false positives or false negatives due to the serializability of transactions. I want to present the theoretical support to justify our methodology. So, the nonce mechanism guarantees serializability? Is a DApp considered a sender? So, what is the mechanism that guarantees transaction serializability for a DApp? That is concurrent transactions sent by a DApp are serializable? https://en.wikipedia.org/wiki/Serializability. I find some web sites mention that blockchain transactions are inherently serializable.}
%\aaron{the nonce guarantees the serializability for transactions from the same sender. Sender should be a user of a DApp, not DApp itself.}
%\aaron{Yes this is what I do in \darcher. Isolate each transaction.}
%\aaron{They are serializable if we consider the whole lifecycle of each transaction. I mean inside the lifecycle, each state transition is like a query or update in concurrent database transaction. If we compare the entire lifecycle to a concurrent database transaction, then they are serializable}
%\aaron{I kind-of understand. You mean DApps are expected to guarantee the serializability of transactions sent by users, and if on-chain-off-chain synchronizaion exists, such serializability may not be achieved?}
To tackle the challenge, we make an observation in on-chain-off-chain synchronization when transactions are executed in isolation, which can be achieved by executing DApp transactions sequentially in \darcher. 
If there is an update to the on-chain state, the off-chain state should change; otherwise the off-chain state should remain unchanged. 
Since the update of the on-chain state depends on the transaction lifecycle states, we can determine whether the off-chain state should change upon traversing the lifecycle states. 
For instance, while the \PendingState state can be visited multiple times, the on-chain state should be the same each time when the state is visited. 
Therefore, the off-chain state should also be the same if the off-chain state is correctly synchronized with the on-chain state.
It means that we do not need to know the mapping $f$ between the on-chain and the off-chain states for the synchronization check at the \PendingState state. 
Instead, we can detect incorrect synchronization by monitoring if there are any changes in the off-chain state each time when the \PendingState is visited. 
%First, DApps are often executed to respect transaction serializability. As such, the logistics of a transaction can be tested in isolation, which is achieved by executing DApp transactions sequentially in \darcher. Second, while the \PendingState state can be visited multiple times, the on-chain state should be the same each time when the state is visited. Therefore, the off-chain state should also be the same if the off-chain state is correctly synchronized with the on-chain state. It means that we do not need the mapping between the off-chain state and the on-chain to check synchronization. Instead, we can detect incorrect synchronization by monitoring if there are any changes in the off-chain state each time when the \PendingState is visited. 
%The same applies to the \ExecutedState state. %^the on-chain state is updated only at the terminal transaction lifecycle states. So, there are no changes to the on-chain state between two visits of the \PendingState state. If As a result, if an DApp's off-chain state differs   observe that the \PendingState and \ExecutedState states in a transaction lifecycle can be visited multiple times. 
%Given that no other transactions modifying the on-chain state are executed between these visits, the \DApp's on-chain state remains the same. 
%Difference of DApp's off-chain states between these visits indicates the inconsistency between the on-chain and the off-chain states. 
% This implies that between these visits，differences in the DApp's off-chain states can indicate the consistency between the on-chain and the off-chain states. 
The observation allows us to propose test oracles for on-chain-off-chain synchronization based only on off-chain states. 
Note that testing transactions in isolation is unlikely to compromise the synchronization bugs that can be detected since most DApps including their centralized database services are executed to respect transaction serializability. %\scc{Have difficulties in following the original writing. Tried to rewrite it based on guessing. Please see if the revised sentences capture the original argument.}
%\aaron{A transaction can revisits a lifecycle state. Between each visit, on-chain states shall remains the same. If off-chain states are not the the same, there might be on-chain-off-chain synchronization bugs in the DApp.}
%\scc{I have further revised the argument. See if it is fine.}
%\aaron{Inspired by Consistency property of databases, I formulate the assertion that DApps should keep during synchronization. Based on the assertion, I add explanations about how the existence of \DroppedState state guides us to design the two oracles. } \scc{Explanation is clearer.}

We make another observation that the \DroppedState state is the key that induces inconsistencies. 
% If there is no \DroppedState state, developers can be sure that the transaction must reach \ConfirmedState state, and on-chain and off-chain states can be easily kept consistent.
Since a transaction can be dropped by the blockchain, a DApp cannot assume that a transaction at the \PendingState state will always transit to the \ConfirmedState state.
%cannot be determined whether there exists some miner that still has $t$ in its mining pool, so 
%As DApps are not able to take any actions when a transaction reaches \DroppedState state.
%\scc{Strictly speaking, the original sentence is incorrect. We should avoid explaining using miner pools unless we want to introduce the concept. So, I rewrote it.}
Since the DApp is not informed of the drop, $\forall i, \sigma_i(t,\PendingState)$ is likely the same as $\sigma(t,\DroppedState)$ when the transaction $t$ is dropped. \scc{Should it be $\sigma_i(t,\PendingState)$? If you find the use of index $i$ cumbersome, we can change it to $\sigma(t,\PendingState)$ referring to the off-chain state at the latest visit of the \PendingState state and $\sigma'(t,\PendingState)$ referring to the one before the latest if the \PendingState state is visited more than once.}\aaron{A typo, my fault}\scc{Do you want to use $\sigma$ and $\sigma'$ without using $\forall$ or keep it as $\sigma_i$ with $\forall$? Either is fine with me but I think the former is less cumbersome.}
If a DApp updates its off-chain state as if the transaction has been finalized when it is still at the \PendingState state, on-chain-off-chain synchronization bugs can occur.

\lili{
1. We may re-emphasize on the challenges in designing automated test oracles that are effective and generic.
2. We may need to explain why we do not simply compare the on-chain and off-chain states as test oracles (This is a simple solution that everyone can think of).
3. Before giving the definitions of the test oracles, we may need to add some intuitions behind them. How they can address the challenges and why they are better than the simple solution.}
\aaron{Put oracles in a separate subsection and emphasize the challenges designing oracles (including why trivial oracle will not work). Intuitions behind oracles are also described.}
%We denote a DApp off-chain state as $\mathbb{S}$, and refer to the off-chain state at each transaction state $s$ of transaction $t$ as $\mathbb{S}(t, s)$. \scc{Why do we use a big capital letter to refer to a state? Cannot follow the meaning of the notation. Looks weird.}
%Due to the fact that whether and when a transaction in the pool will be executed is non-deterministic, we design our first oracle at \PendingState state of a transaction:
%A transaction may either make a query that does not change the DApp's on-chain state or an update that modifies the on-chain state. 

\scc{It looks more like an assertion than an oracle.}
\aaron{I am confused. Do you mean we should say we propose two ``assertions'' instead of ``oracles''?} \scc{Strictly speaking, the oracle should be checking whether the assertion is fulfilled and how/when the checking is made based on the proposed traversal order. That said, the current form is also fine. If you rename it to assertion, add a couple of sentences explaining the test oracle.}
\aaron{I see. If current form is fine, let's keep it.}

%\scc{The second oracle seems to require $\sigma$ and $\sigma'$. The current version $\sigma_t(Pending)$ should be the same is weird. Mathematically, $\sigma_t(Pending)$ should map to one value but we are using it to map to different values non-deterministically. If so, we need to refine Oracle 1 with there exists and for all mapped values.}
%\aaron{How about we don't put formulation, and only explain the oracle in a few sentences? I check the oracles proposed by ContractFuzzer~\cite{contractfuzzer}, and they don't use formulations, e.g. ``The first sub-oracle is \textbf{TimestampOp} that checks whether the calls within the current contract have invoked the TIMESTAMP opcode during execution.''} \scc{I made a fix. See if it is fine with you. }
%\scc{Also, it seems that the oracle applies to the outcomes of one test rather than multiple tests. I don't think it is a metamorphic relation.}\aaron{OK, so let us do not mention metamorphic relation.}
%\aaron{They look good. Thank you.}

%Oracles for on-chain-off-chain synchronization bugs are introduced as follows:
Here, let us formulate the test assertion for the Type-I bugs as shown in Fig.~\ref{fig:bug-diagram}(a). %the DApp assumes a \PendingState transaction $t$ will transit into the \ConfirmedState state and prematurely updates the off-chain state.
As the transaction is dropped, there is no update to the on-chain state, i.e., $\mu(t,\DroppedState) = \mu(t,\CreatedState)$.
Since $\sigma(t,\CreatedState)=f(\mu(t,\CreatedState))$ and $\sigma(t,\DroppedState)=f(\mu(t,\DroppedState))$, $\sigma(t,\CreatedState) = \sigma(t,\DroppedState)$.
As explained, a DApp is usually unaware of that a transaction has been dropped.
As a result, updates, if any, to the off-chain state at the \PendingState state will remain, i.e., $\forall i$, chances are that $\sigma_i(t, \PendingState) = \sigma(t, \DroppedState)$. \scc{Should we care only the last $i$?}
Therefore, We formulate the assertion for Type-I bug as $\forall i, \sigma_i(t,\PendingState) \neq \sigma(t,\CreatedState)$.
Nevertheless, the assertion is too strict. \scc{I cannot follow the reasoning between the last statement and the next statement and how $\forall i, \sigma_i(t,\PendingState) \neq \sigma(t,\CreatedState)$ becomes $\sigma(t,\DroppedState) \neq \sigma(t,\ConfirmedState)$.}
A necessary condition for correct synchronization of an update transaction is $\sigma(t,\DroppedState) \neq \sigma(t,\ConfirmedState)$. 
As a result, the assertion can be rewritten as $\forall i, \sigma_i(t,\PendingState) \neq \sigma(t,\ConfirmedState)$. 
% because DApps may \textit{partially} update the off-chain state when transaction is \PendingState to improve user experience, e.g.,\ add a label indicating that the transaction is \PendingState.
% So we relax the assertion and propose the following oracles. 
%\scc{I cannot follow the relaxation? The explanation sounds confusing. }
\aaron{Now I only say we use a necessary condition to define oracles. See if it is fine.}\scc{The logic is confusing. In the beginning, we introduce an assertion whose satisfaction indicates that bug occurs, and then we relax this assertion to formulate an assertion whose violation indicates that bug occurs. I prefer this logic: When a \ConfirmedState transaction results in an update to on-chain state, $\sigma(t,\CreatedState) \neq \sigma(t,\ConfirmedState)$ is a necessary condition for correct synchronization. On the other hand, if the transaction is dropped, $\sigma(t,\DroppedState) = \sigma(t,\CreatedState)$ is a necessary condition for correct synchronization. Therefore, a necessary condition for correct synchronization of such a transaction is $\sigma(t,\DroppedState) \neq \sigma(t,\ConfirmedState)$. Since an DApp is not informed of the transaction drop, $\sigma(t,\DroppedState) = \sigma(t,\PendingState)$. As a result, the necessary condition can be rewritten as $\sigma(t,\PendingState) \neq \sigma(t,\ConfirmedState)$. Also, I think we care only the last $i$.}

\begin{oracle}
    \label{oracle1}
    For each transaction $t$,
    $\sigma(t,\CreatedState) \neq \sigma(t,\ConfirmedState)$ implies $ \forall i,  \sigma_i(t,\PendingState) \neq \sigma(t,\ConfirmedState)$.
\end{oracle}

The clause $\sigma(t,\CreatedState) \neq \sigma(t,\ConfirmedState)$ characterizes a transaction that results in an update. 
The clause $\sigma_i(t,\PendingState) \neq \sigma(t,\ConfirmedState)$ specifies that at least part of the update should be taken when the transaction transits from \PendingState to \ConfirmedState, so that $\sigma(t,\DroppedState)$ could at least differ from $\sigma(t,\ConfirmedState)$ and the DApp can tell that the transaction is not \ConfirmedState.
%If $\sigma(t,\CreatedState) \neq \sigma(t,\ConfirmedState) \land \exists i, 
%\sigma_i(t,\PendingState) = \sigma(t, \ConfirmedState)$, it indicates that all the off-chain state update that is expected to make according to the transaction has been done, in some visit of \PendingState state. 
Violation of the clause means $\exists i, \sigma_i(t,\PendingState) = \sigma(t, \ConfirmedState)$. 
Since $\sigma(t,\CreatedState) \neq \sigma(t,\ConfirmedState)$, the violation indicates that the off-chain state has sometimes been prematurely updated when the transaction is at the \PendingState state. 
%If such scenario happens, the DApp's off-chain state would be updated as if the transaction is executed, while it is actually still in the \PendingState state.
It therefore reveals a Type-I on-chain-off-chain synchronization bug in the DApp.
%We use the \PendingState state because it is the point that introduces non-determinism in transaction. 
%\scc{The justification of \PendingState can be strengthened. I cannot follow your original explanation, which seems a bit confusing. So, I rewrote it. See if it is fine.} 
%\aaron{I revise the explanation. Please check if it makes sense.} \scc{Not really follow. Why is $\sigma(t,\PendingState) \neq \sigma(t,\ConfirmedState)$ related to \CreatedState? The clause does not contain \CreatedState. Why does this clause indicate that "the DApp assumes ..."? I seem to have missed some implicit assumptions in your argument.}
%\aaron{Updated.} \scc{There are writing mistakes. I rewrote it. See if it is fine.}\aaron{Thanks.}
%In the current \darcher implementation, the data fields that contribute to an off-chain state are specified by the test engineers.

%Oracle~\ref{oracle1} states that off-chain state at transaction \PendingState state should be distinguishable compared to that at \ConfirmedState state, if the DApp is intended to make modifications according to the transaction.
%The intuition behind is that a transaction being put in the transaction pool (i.e.~at \PendingState state) is not a guarantee of being confirmed eventually.
%Therefore, DApp off-chain state should not be modified as if the transaction is confirmed, i.e.~DApp state at \PendingState should not be the same as \ConfirmedState state.
%Condition $\mathbb{S}(t, \CreatedState) \neq \mathbb{S}(t, \ConfirmedState)$ states that this oracle is only applied when there are some differences in DApp state between \CreatedState and \ConfirmedState, which indicates the DApp is intended to make some modification according to the transaction.
%Otherwise, this oracle does not need to be applied because the DApp is not designed to do anything according to this transaction.

Let us consider scenario in Type-II bugs. 
When a transaction is executed, it transits from the \PendingState to the \ExecutedState state, where some DApps may pre-maturely update their off-chain state. 
However, such updates need to be unrolled if the transaction is reserved to the \PendingState state upon chain reorganization, because the reversed transaction may get dropped silently.
We, therefore, formulate it with the following test oracle.

\begin{oracle}
    \label{oracle2}
    For each transaction $t$, $\forall i \forall j, \sigma_i(t,\PendingState) = \sigma_j(t,\PendingState)$. 
\end{oracle}

%The intuition behind is that there is still possibility an executed transaction can be removed from blockchain history and return back to \PendingState state due to blockchain reorganization.
%After returning to \PendingState state, the transaction still has the chance to go to \DroppedState state.
%It is non-deterministic whether a removed transaction can be re-executed again or not.
%If DApp state is modified when transaction reaching \ExecutedState state from \PendingState state, when the transaction goes back to \PendingState state, it should be reverted so that off-chain state is consistent with on-chain state of DApp.
%On-chain state has been reverted to the state when transaction is \PendingState, and so should the off-chain state.

%When the transaction is being processed by blockchain cluster, at each transaction state, \darcher will fetch off-chain state of DApp according to manual specifications.
%Base on the off-chain state of DApps on each transaction state, \darcher is able to perform an offline analysis using the proposed oracles.
%For each transaction, if the oracles are violated, which indicates off-chain state is not consistent with on-chain state of DApp at a specific transaction state, bug reports will be generated for this transaction and help developers locate the on-chain-off-chain synchronization bug.
%An on-chain-off-chain synchronization bug is detected if any of the two above test assertions is violated.


==> 6-Evaluation/baseline-results.table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
    \centering
    \caption{Experiment Results of Baseline Methods \scc{I think the performance of baseline and \darcher should be put in the same table.}}
    \label{tab:baseline-results}
    \begin{threeparttable}
        \begin{tabular}{@{}c|c|c|cc|c@{}}
            \toprule
            \multirow{3}{*}{DApp} & \multirow{2}{*}{Vul.\tnote{1}} & \multicolumn{3}{c|}{Transaction Failures}
            & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
                                  Runtime\\ Errors
            \end{tabular}} \\ \cmidrule(lr){3-5}
            & & Txs.\tnote{2} & \multicolumn{2}{c|}{Func.\tnote{3}} & \\ \cmidrule(l){2-6}
            & Avg.\tnote{4} & \multicolumn{1}{l|}{Avg.} & \multicolumn{1}{l}{Aggr.\tnote{5}} & Avg. & Avg.   \\ \midrule
            AgroChain              & 0    & 0                         & 0                         & 0    & 437.3  \\
            Augur                  & 0    & 0                         & 0                         & 0    & 354.9  \\
            burner-wallet          & 0    & 0                         & 0                         & 0    & 3743.1 \\
            DemocracyEarth         & 0    & 19.9                      & 1                         & 1    & 54.3   \\
            eth-hot-wallet         & 0    & 0                         & 0                         & 0    & 1612.4 \\
            ethereum\_voting\_dapp & 0    & 23..6                     & 1                         & 1    & 909.6  \\
            ethereum-todolist      & 0    & 0                         & 0                         & 0    & 360.6  \\
            Giveth                 & 0    & 0                         & 0                         & 0    & 113.0  \\
            Heiswap                & 0    & 1.3                       & 1                         & 0.5  & 307.5  \\
            MetaMask               & 0    & 0.3                       & 1                         & 0.2  & 3012.2 \\
            Multisender            & 0    & 0                         & 0                         & 0    & 242.0  \\
            publicvotes            & 0    & 0                         & 0                         & 0    & 827.9  \\ \bottomrule
        \end{tabular}%
        \begin{tablenotes}
            \item[1] Vul.~is short for Contract Vulnerabilities. \scc{Is the format too space wasting?}

            \item[2] Txs.~is short for Transactions.

            \item[3] Func.~is short for Functionalities.

            \item[4] Avg.~is short for Averaged.

            \item[5] Aggr.~is short for Aggregated.
        \end{tablenotes}
    \end{threeparttable}
\end{table}


==> formalization.tex <==
% \section{Formalization}

% % We can regard a DApp with on-chain and off-chain state as a whole as a hyper-database and define \textit{hyper-transaction} that this hyper-database executes. 
% % A DApp, including on-chain and off-chain layer, executes a hyper-transaction by validating user input, create blockchain transactions, submit transaction to blockchain and update off-chain state accordingly when blockchain transaction has been executed. 
% % Hyper-transaction is submitted when blockchain is submitted to blockchain.
% % Hyper-transaction commits when the corresponding blockchain transaction is finalized. 
% % Hyper-database need to have ACID properties as 

% We use $\mu(t,s)$ and $\sigma(t,s)$ to denote a DApp's on-chain and off-chain state in transaction $t$ at lifecycle state $s$, respectively. 
% As a transaction can visit \PendingState and \ExecutedState multiple times, we use $\mu_i(t,s)$ and $\sigma_i(t,s)$ to denote the on-chain and off-chain state when the transaction $t$ makes the $i^{th}$ visit of \PendingState or \ExecutedState state, respectively.
% We use $f$ to denote the mapping between on-chain and off-chain state. 
% The consistency of on-chain and off-chain state can be represented as 


% \begin{equation} \label{eq1}
% \begin{split}
%     \sigma(t, \CreatedState) &\equiv f(\mu(t, \CreatedState)) \\
%     &\land \\
%     \sigma(t, \ConfirmedState) &\equiv f(\mu(t, \ConfirmedState)) 
% \end{split}
% \end{equation}



==> terminologies.tex <==
\section{Terminologies}

I found we have many inconsistencies in the terminologies we use in the paper. 
So I create this file to clarify the terminologies we should use consistently.
I will try my best to find the terminologies used by literature or communities. 
Please check this file from time to time so that we can keep the terminologies in our writing consistent.

\subsection{Blockchain and Transaction}

\begin{itemize}
    \item \textbf{Chain reorganization}: 
        We use ``chain reorganization'' instead of ``blockchain reorganization''.\footnote{https://en.bitcoin.it/wiki/Chain\_Reorganization}
    \item Transaction is \textbf{executed}
        ``Execute'' refers to the action where the transaction is included in the block. 
        It is used in the very first Bitcoin paper by Nakamoto~\cite{bitcoin}.
    \item Transaction is \textbf{reversed}:
        Gervais et al.~\cite{security_and_performance_of_PoW} uses ``reverse'' when saying ``The more confirmations a transaction obtains, the less likely this transaction will be reversed in the future.''
    \item Transaction is \textbf{dropped}:
        ``Drop'' means the transaction is deleted by miners from transaction pool. \footnote{https://info.etherscan.com/transaction-dropped-replaced/}
    % \item We should use \textbf{mining pool} instead of transaction     pool~\cite{whitepaper}\footnote{https://ethereum.org/en/whitepaper/\#mining-centralization}
\end{itemize}


